Graph Message Passing with Cross-location Attentions for Long-term ILI Prediction

Forecasting influenza-like illness (ILI) is of prime importance to epidemiologists and health-care providers. Early prediction of epidemic outbreaks plays a pivotal role in disease intervention and control. Most existing work has either limited long-term prediction performance or lacks a comprehensive ability to capture spatio-temporal dependencies in data. Accurate and early disease forecasting models would markedly improve both epidemic prevention and managing the onset of an epidemic. In this paper, we design a cross-location attention based graph neural network (Cola-GNN) for learning time series embeddings and location aware attentions. We propose a graph message passing framework to combine learned feature embeddings and an attention matrix to model disease propagation over time. We compare the proposed method with state-of-the-art statistical approaches and deep learning models on real-world epidemic-related datasets from United States and Japan. The proposed method shows strong predictive performance and leads to interpretable results for long-term epidemic predictions.

==> sections/more_results.tex <==
\onecolumn
\section{Supplemental Material}
 \subsection{More results 1}
 
In addition to the results in the paper, we evaluate the proposed method compared to other state-of-the-art methods for a shorter leadtime. Table~\ref{table:extra-rmse-pcc} demonstrates the prediction results for leadtime = 2,3 and 4 weeks.
  All experimental results are the average of 10 randomized trials (10 fixed random seeds for all models).  

 \begin{table*}[h]
\footnotesize
\centering
\vspace{-1em}
\scalebox{0.95}{\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{\textbf{Japan-Prefectures}} & \multicolumn{3}{c}{\textbf{US-Regions}} & \multicolumn{3}{c}{\textbf{US-States}} \\
\cmidrule(r){2-4}\cmidrule(r){5-7}\cmidrule(r){8-10}
\textbf{RMSE($\downarrow$)} & 2 & 3  & 4 & 2 & 3  & 4 & 2 & 3  & 4 \\
\hline
GAR & 1486  & 1991  & 2282 & 607& 792  & 934  & 162  &200 & 221  \\
AR &  1669 & 2071  & 2313 & 623 &812 & 955  & 172  & 212  & 242  \\
VAR &  1585 & 2105  & 2451 & 697 &859 &  988 & 294  & 287  &  313 \\
ARMA & 1662  &  2070 & 2312 & 623 & 805 & 939  & 172  &183  &  240 \\
RNN &  1191 &1562 & 1714 &573 &752 & 880 & 160 & 196  & 211 \\
RNN+Attn & 1444  & 1682  &2038 &847 & 1204  &879   &  163  & 213 & 234 \\
CNNRNN-Res & 1302  & 1719  & 1904&618 & 780  & 871  & 200   & 241 & 250 \\
GCNRNN-Res & 1207 &  1472 &1614 &735 &  853 &  896 &  215  & 238 & 245\\
Cola-GNN & \textbf{1162}   & \textbf{1378} & \textbf{1522} &\textbf{544} &\textbf{708}   & \textbf{804}  &   \textbf{147} &  \textbf{172} & \textbf{187} \\
\midrule

\textbf{PCC($\uparrow$)} & 2 & 3  & 4 & 2 & 3  & 4 & 2 & 3  & 4 \\
\midrule
GAR &  0.8022 &  0.6129 &0.4438 &   0.9236  &0.87 & 0.823 & 0.9381 & 0.9055 & 0.8839 \\
AR &  0.7429 &  0.567  & 0.4127 & 0.9217 & 0.8709 &0.8291 &  0.9335 &  0.9019  & 0.8742 \\
VAR & 0.7688 &  0.5627  & 0.3667 & 0.8947 & 0.8411 & 0.7818 &  0.7869  & 0.7970  &  0.7555 \\
ARMA &   0.7446 & 0.5672  & 0.4135 & 0.9202& 0.8701 &  0.8275 & 0.9322   & 0.9253 & 0.8729 \\
RNN & 0.8879 & 0.806 & 0.7835 & 0.9339&0.8867 & 0.8499 & 0.9434  &0.9142  & 0.8997 \\
RNN+Attn &  0.7955  &  0.7473 & 0.6143 & 0.8123& 0.6801 &  0.8526 &  0.9422  &  0.8961 &  0.8679\\
CNNRNN-Res &  0.863 &  0.7233  &0.6473  & 0.92 & 0.8689&  0.8307 & 0.9115   &  0.8699  & 0.8492 \\
GCNRNN-Res &  0.8925  & 0.8323 & 0.8101 & 0.8979&   0.8638&  0.8456 &  0.8893  & 0.8617 &  0.8576\\
Cola-GNN &  \textbf{0.8928} &  \textbf{0.859}  & \textbf{0.8298} & \textbf{0.9397} &\textbf{0.9003} &   \textbf{0.8681} &   \textbf{0.9516} & \textbf{0.9347} & \textbf{0.9269}\\
\bottomrule
\end{tabular}}
\caption{RMSE and PCC performance of different methods on the three datasets with leadtime= 2, 3, 4. Bold face indicates the best result of each column. We follow the same experimental setup mentioned in the paper.}\label{table:extra-rmse-pcc}
\end{table*}
 
\vspace{-1em}
 \subsection{More results 2}
We further evaluate these methods by changing the training-validation-testing split setting to 50\%-20\%-30\%. The test sets include more flu seasons. Table~\ref{table:extra2-rmse-pcc} shows the prediction results for leadtime = 2 and 5 weeks.
 
  \begin{table*}[h]
\footnotesize
\centering
\vspace{-1em}
\scalebox{0.95}{\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Japan-Prefectures}} & \multicolumn{2}{c}{\textbf{US-Regions}} & \multicolumn{2}{c}{\textbf{US-States}} \\
\cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}
\textbf{RMSE($\downarrow$)} & 2 & 5   & 2 & 5   & 2 & 5   \\
\hline
GAR &  1232 & 1988   &  536  &  991  & 150  & 236 \\
AR & 1377  &  2013  &   571 &  997  &  290 & 295 \\
VAR & 1361  & 2025  &  741  & 1059   & 290  & 295 \\
ARMA & 1371 &  2013  &  560  &  989  &  161 & 250 \\
RNN & 1001  &  1375   &  513  & 896   &  149 & 217\\
RNN+Attn & 1166 & 1746   &   613  & 1065   & 152  & 234 \\
CNNRNN-Res & 1133 & 1942   & 571   & 936   &  205 & 268  \\
GCNRNN-Res & 1031 & 1178   &  736  & 1051   &  194 & 248\\
Cola-GNN &  \textbf{957} &  \textbf{1168}  & \textbf{483}   &  \textbf{871}  & \textbf{137}  & \textbf{211}\\
\midrule

\textbf{PCC($\uparrow$)} & 2 & 5  & 2 & 5 & 2  & 5   \\
\midrule
GAR &  0.8042  &  0.3389  &  0.9318  & 0.7902   & 0.9445  &  0.8746  \\
AR & 0.752  &  0.3095  &  0.9273  & 0.7923   &  0.7649 & 0.7584 \\
VAR & 0.7537 &  0.2995  &  0.8586  &  0.6853  & 0.7649  & 0.7584 \\
ARMA & 0.754  & 0.3102   &  0.9265  & 0.7922   & 0.9387  & 0.8621 \\
RNN & 0.892 &  0.8207  &  0.9404  & 0.8206   & 0.9484  &  \textbf{0.8862}\\
RNN+Attn & 0.8498  &  0.589  & 0.8874 &  0.7524  & 0.9472  & 0.8836\\
CNNRNN-Res & 0.8524 & 0.3804   &  0.9196  &  0.7817  & 0.9036  &0.8222 \\
GCNRNN-Res &  0.8928 &  0.8748  & 0.8711   &  0.7385  & 0.9029  & 0.844\\
Cola-GNN &  \textbf{0.9012} & \textbf{0.8793}   &  \textbf{0.9438}  &   \textbf{0.8324} &  \textbf{0.954} & 0.8825 \\
\bottomrule
\end{tabular}}
\caption{RMSE and PCC performance of different methods on the three datasets with leadtime= 2, 5.}
\label{table:extra2-rmse-pcc}
\end{table*}
 
 \subsection{Model Complexity Analysis}
Table~\ref{complexity} shows the comparison of runtimes and numbers of parameters for each model on the US-States dataset, which has the  largest number of \textit{regions} among the three datasets.
 \begin{table}[h]
\small
\centering
% \vspace{-1em}
\begin{tabular}{lrc}
\toprule
\textbf{Architecture}    & \textbf{Parameters}  & \textbf{Runtime(s)}  \\
\midrule
GAR      &     21        &  0.01           \\ 
AR      &      1,029    &   0.02 \\ 
VAR      &     48,069        &  0.02  \\ 
ARMA      &      1,960 & 0.03          \\ 
RNN      &     481       &   0.04   \\ 
RNN+Attn   &  1,321    &    0.58 \\
CNNRNN-Res   &    7,695    &  0.04     \\
GCNRNN-Res    &    6,214     &  0.04      \\
Cola-GNN  &    3,778    &    0.21     \\
\bottomrule
\end{tabular}
\caption{Runtime comparison of models on the  US-States dataset. Runtime is the time spent on a single GPU per epoch.}
\label{complexity}
\end{table}


\subsection{More visual results}
We provide more visual results of these three datasets in Figure~\ref{fig:more-leadtime-curves}. We fixed the input window and plotted the lead time prediction curve from 1 to 20. The numerical values are collected from models that trained on the same experimental setting in this paper.
  \begin{figure}[h]
  \centering 
  
   \begin{subfigure}[b]{.68\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/legend.pdf}
  \end{subfigure} 
     \hspace{-5pt}
     
    \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-Japan-Tokushima.pdf}
  \end{subfigure} 
     \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-Japan-Kagawa.pdf}
  \end{subfigure} 
    \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-Japan-Kanagawa.pdf}
  \end{subfigure} 
   \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-Japan-Yamanashi.pdf}
  \end{subfigure} 
   \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-Japan-Shimane.pdf}
  \end{subfigure} 
   \hspace{-5pt}
    \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Region1.pdf}
    %  \subcaption{US-Regions}\label{fig:region-window}
  \end{subfigure} 
  \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Region2.pdf}
    %  \subcaption{US-States}\label{fig:state-window}
  \end{subfigure} 
    \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Region6.pdf}
    %  \subcaption{US-States}\label{fig:state-window}
  \end{subfigure} 
    \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Region7.pdf}
    %  \subcaption{US-States}\label{fig:state-window}
  \end{subfigure} 
    \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Region8.pdf}
    %  \subcaption{US-States}\label{fig:state-window}
  \end{subfigure} 
    \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Colorado.pdf}
  \end{subfigure} 
     \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Hawaii.pdf}
  \end{subfigure} 
    \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-Massachusetts.pdf}
  \end{subfigure} 
   \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-NewJersey.pdf}
  \end{subfigure} 
    \hspace{-5pt}
  \begin{subfigure}[b]{.2\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{figures/more-curves-US-NorthDakota.pdf}
  \end{subfigure} 
  \caption{Direct prediction curves with fixed input windows.}
  \label{fig:more-leadtime-curves}
 \end{figure}

==> tables/ablation-pcc+rmse.tex <==
% \begin{table}[t]
% \centering
% \footnotesize
% \caption{Ablation test results in RMSE(top) and PCC(bottom) when leadtime=1,5,10,15 for three datasets.}\label{ablation-rmse-pcc}
% \begin{tabular}{|r|cccc|}
% \hline
% \cellcolor{grey!10} \textbf{RMSE($\downarrow$)}  & \multicolumn{4}{c|}{Japan-Prefectures} \\
% Methods & 1 & 5 & 10 & 15  \\
% \hline
% Ours-temp &  713 &  1698 & \underline{1816}  & 1931  \\ 
% Ours-loc &  \textbf{697} & \underline{1588} & 1867  & \underline{1767}  \\  
% Ours &  \underline{710}  &  \textbf{1553} & \textbf{1754} & \textbf{1638}   \\
% \hline
%  & \multicolumn{4}{c|}{US-Regions}  \\
% % Methods & 1 & 5 & 10 & 15  \\
% \hline
% Ours-temp  &  \textbf{341} & \underline{878}  &  \underline{989} & \underline{983}   \\ 
% Ours-loc  &  348 &  930  & 1152  & 1200   \\  
% Ours &  \underline{342}  & \textbf{874}  & \textbf{953}  &  \textbf{949} \\
% \hline
%  & \multicolumn{4}{c|}{US-States} \\
% % Methods & 1 & 5 & 10 & 15  \\
% \hline
% Ours-temp &  \textbf{106} &  \underline{208} &  \underline{240} & \underline{251}  \\ 
% Ours-loc &   \underline{108} &  218   & 266  & 281   \\  
% Ours &  \textbf{106}  & \textbf{203}  &  \textbf{228} & \textbf{229}  \\
% \hline
% \hline
% \cellcolor{grey!10} \textbf{PCC($\uparrow$)} & \multicolumn{4}{c|}{Japan-Prefectures}  \\
% Methods & 1 & 5 & 10 & 15  \\
% \hline
% Ours-temp &  0.9608 & 0.7593  & 0.7623  & 0.6895    \\ 
% Ours-loc & \textbf{0.9645}  & \textbf{0.8532}  & \underline{0.7753}  &  \underline{0.7806}   \\ 
% Ours & \underline{0.9622} & \underline{0.84} & \textbf{0.7982} &  \textbf{0.7922}  \\
% \hline
%  & \multicolumn{4}{c|}{US-Regions} \\
% % Methods & 1 & 5 & 10 & 15 \\
% \hline
% Ours-temp & \textbf{0.9763} & \underline{0.847}  & \underline{0.8175}  &  \textbf{0.8146} \\ 
% Ours-loc&  0.9755 & 0.842  & 0.7857  &  0.7811 \\ 
% Ours  &  \underline{0.976} &  \textbf{0.8548} & \textbf{0.8201}  & \underline{0.8135}  \\
% \hline
%  &  \multicolumn{4}{c|}{US-States} \\
% % Methods & 1 & 5 & 10 & 15  \\
% \hline
% Ours-temp & \textbf{0.9745} & \underline{0.9101}  & \underline{0.8801} & \underline{0.8796}  \\ 
% Ours-loc & 0.9739  &0.905   & 0.866  &0.8734     \\ 
% Ours &  \textbf{0.9745} &  \textbf{0.9121} & \textbf{0.8932} & \textbf{0.8927} \\
% \hline
% \end{tabular}
% \label{tbl:ablation-rmse}
% \end{table}


\begin{table}[t]
\centering
\footnotesize
\caption{Ablation test results in RMSE(top) and PCC(bottom) when leadtime=1,5,10,15 for three datasets.}\label{ablation-rmse-pcc}
\scalebox{1.0}{\begin{tabular}{lcccc}
\toprule
% \multicolumn{5}{|c|}{\cellcolor{grey!10} \textbf{RMSE($\downarrow$)}} \\
% \rowcolor{grey!10}
\textbf{RMSE($\downarrow$)} & 1 & 5 & 10 & 15  \\
\midrule
& \multicolumn{4}{c}{Japan-Prefectures} \\
\cmidrule(r){2-5}
Cola-GNN-$temp$ &  713 &  1698 & \underline{1816}  & 1931  \\ 
Cola-GNN-$loc$ &  \textbf{697} & \underline{1588} & 1867  & \underline{1767}  \\
Cola-GNN &  \underline{710}  &  \textbf{1553} & \textbf{1754} & \textbf{1638}   \\
\midrule
& \multicolumn{4}{c}{US-Regions}  \\
% Methods & 1 & 5 & 10 & 15  \\
\cmidrule(r){2-5}
Cola-GNN-$temp$  &  \textbf{341} & \underline{878}  &  \underline{989} & \underline{983}   \\ 
Cola-GNN-$loc$  &  348 &  930  & 1152  & 1200   \\  
Cola-GNN &  \underline{342}  & \textbf{874}  & \textbf{953}  &  \textbf{949} \\
\midrule
& \multicolumn{4}{c}{US-States} \\
% Methods & 1 & 5 & 10 & 15  \\
\cmidrule(r){2-5}
Cola-GNN-$temp$ &  \textbf{106} &  \underline{208} &  \underline{240} & \underline{251}  \\ 
Cola-GNN-$loc$ &   \underline{108} &  218   & 266  & 281   \\  
Cola-GNN &  \textbf{106}  & \textbf{203}  &  \textbf{228} & \textbf{229}  \\
\midrule
% \multicolumn{5}{|c|}{\cellcolor{grey!10} \textbf{PCC($\downarrow$)}} \\
% Methods & 1 & 5 & 10 & 15  \\
% \rowcolor{grey!10}
\textbf{PCC($\uparrow$)} & 1 & 5 & 10 & 15  \\
\midrule
% \cellcolor{grey!10} \textbf{PCC($\uparrow$)} & \multicolumn{4}{c|}{Japan-Prefectures}  \\
% Methods & 1 & 5 & 10 & 15  \\
& \multicolumn{4}{c}{Japan-Prefectures} \\
\cmidrule(r){2-5}
Cola-GNN-$temp$ &  0.9608 & 0.7593  & 0.7623  & 0.6895    \\ 
Cola-GNN-$loc$ & \textbf{0.9645}  & \textbf{0.8532}  & \underline{0.7753}  &  \underline{0.7806}   \\ 
Cola-GNN & \underline{0.9622} & \underline{0.84} & \textbf{0.7982} &  \textbf{0.7922}  \\
\midrule
& \multicolumn{4}{c}{US-Regions} \\
% Methods & 1 & 5 & 10 & 15 \\
\cmidrule(r){2-5}
Cola-GNN-$temp$ & \textbf{0.9763} & \underline{0.847}  & \underline{0.8175}  &  \textbf{0.8146} \\ 
Cola-GNN-$loc$&  0.9755 & 0.842  & 0.7857  &  0.7811 \\ 
Cola-GNN  &  \underline{0.976} &  \textbf{0.8548} & \textbf{0.8201}  & \underline{0.8135}  \\
\midrule
& \multicolumn{4}{c}{US-States} \\
% Methods & 1 & 5 & 10 & 15  \\
\cmidrule(r){2-5}
Cola-GNN-$temp$ & \textbf{0.9745} & \underline{0.9101}  & \underline{0.8801} & \underline{0.8796}  \\ 
Cola-GNN-$loc$ & 0.9739  &0.905   & 0.866  &0.8734     \\ 
Cola-GNN &  \textbf{0.9745} &  \textbf{0.9121} & \textbf{0.8932} & \textbf{0.8927} \\
\bottomrule
\end{tabular}}
\label{tbl:ablation-rmse}
\end{table}

==> tables/ablation-pcc.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{\footnotesize Ablation test results in PCC}
\begin{tabular}{|r|cccc|}
\hline
 & \multicolumn{4}{c|}{Japan-Prefectures}  \\
\rowcolor{grey!10}Methods & 1 & 5 & 10 & 15  \\
\hline
Ours-temp &  0.9608 & 0.7593  & 0.7623  & 0.6895    \\ 
Ours-loc & 0.9645  & 0.8532  & 0.7753  &  0.7806   \\ 
Ours & 0.9622 & 0.84 & \textbf{0.7982} &  \textbf{0.7922}  \\
\hline
 & \multicolumn{4}{c|}{US-Regions} \\
\rowcolor{grey!10}Methods & 1 & 5 & 10 & 15 \\
\hline
Ours-temp & 0.9763& 0.847  & 0.8175  &  0.8146 \\ 
Ours-loc&  0.9755 & 0.842  & 0.7857  &  0.7811 \\ 
Ours  &  \underline{0.976} &  \textbf{0.8548} & \textbf{0.8201}  & \underline{0.8135}  \\
\hline
 &  \multicolumn{4}{c|}{US-States} \\
\rowcolor{grey!10}Methods & 1 & 5 & 10 & 15  \\
\hline
Ours-temp & 0.9745 & 0.9101  & 0.8801 & 0.8796  \\ 
Ours-loc & 0.9739  &0.905   & 0.866  &0.8734     \\ 
Ours &  \underline{0.9745} &  \textbf{0.9121} & \textbf{0.8932} & \textbf{0.8927} \\
\hline
\end{tabular}
\label{tbl:ablation-pcc}
\end{table}


% \begin{table*}[]
% \small
% \caption{Ablation test results in PCC}
% \begin{tabular}{|r|cccc|cccc|cccc|}
% \hline
%  & \multicolumn{4}{c|}{Japan-Prefectures} & \multicolumn{4}{c|}{US-Regions} & \multicolumn{4}{c|}{US-States} \\
% Methods & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 \\
% \hline
% Ours-temp &  0.9608 & 0.7593  & 0.7623  & 0.6895  & 0.9763& 0.847  & 0.8175  &  0.8146&  0.9745 & 0.9101  & 0.8801 & 0.8796  \\ 
% Ours-loc & 0.9645  & 0.8532  & 0.7753  &  0.7806 &  0.9755 & 0.842  & 0.7857  &  0.7811 & 0.9739  &0.905   & 0.866  &0.8734     \\ 
% Ours & 0.9622 & 0.84 & \textbf{0.7982} &  \textbf{0.7922} &  \underline{0.976} &  \textbf{0.8548} & \textbf{0.8201}  & \underline{0.8135}  &  \underline{0.9745} &  \textbf{0.9121} & \textbf{0.8932} & \textbf{0.8927} \\
% \hline
% \end{tabular}
% \label{tbl:ablation-pcc}
% \end{table*}

==> tables/ablation-rmse.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{\footnotesize Ablation test results in RMSE}
\begin{tabular}{|r|cccc|}
\hline
 & \multicolumn{4}{c|}{Japan-Prefectures} \\
\rowcolor{grey!10}Methods & 1 & 5 & 10 & 15  \\
\hline
Ours-temp &  713 &  1698 & 1816  & 1931  \\ 
Ours-loc &  697 & 1588 & 1867  & 1767  \\  
Ours &  710  &  \textbf{1553} & \textbf{1754} & \textbf{1638}   \\
\hline
 & \multicolumn{4}{c|}{US-Regions}  \\
\rowcolor{grey!10}Methods & 1 & 5 & 10 & 15  \\
\hline
Ours-temp  &  341 & 878  &  989 & 983   \\ 
Ours-loc  &  348 &  930  & 1152  & 1200   \\  
Ours &  \underline{342}  & \textbf{874}  & \textbf{953}  &  \textbf{949} \\
\hline
 & \multicolumn{4}{c|}{US-States} \\
\rowcolor{grey!10}Methods & 1 & 5 & 10 & 15  \\
\hline
Ours-temp &  106 &  208 &  240 & 251  \\ 
Ours-loc &   108 &  218   & 266  & 281   \\  
Ours &  \underline{106}  & \textbf{203}  &  \textbf{228} & \textbf{229}  \\
\hline
\end{tabular}
\label{tbl:ablation-rmse}
\end{table}

% \begin{table*}[]
% \small
% \caption{Ablation test results in RMSE}
% \begin{tabular}{|r|cccc|cccc|cccc|}
% \hline
%  & \multicolumn{4}{c|}{Japan-Prefectures} & \multicolumn{4}{c|}{US-Regions} & \multicolumn{4}{c|}{US-States} \\
% Methods & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 \\
% \hline
% % Ours-$loc$-$temp$ & \textbf{695}  &  1593 & \textbf{1754}  & \underline{1748}  &  344 & \textbf{866}  & 1046  &  1124 &  \textbf{105} & 204  & 256  & 267  \\ 
% Ours-temp &  713 &  1698 & 1816  & 1931  &  341 & 878  &  989 & 983  & 106 &  208 &  240 & 251  \\ 
% Ours-loc &  697 & 1588 & 1867  & 1767  &  348 &  930  & 1152  & 1200  &    108 &  218   & 266  & 281   \\  

% %  Ours-$loc$-$temp$& \textbf{684}  & 1602  & 1931  &  \underline{1729} &  \textbf{337} & \textbf{860}  &  \underline{1078} &  \underline{1196} & \textbf{102}   & \textbf{203}  &  \underline{249} & \underline{264}  \\
% % Ours-$loc$ & \underline{697}  & \underline{1597}  & \underline{1867}  &  1767 &  348 & 941  & 1152  & 1226  &  108 & \underline{218}  & 266  & 281  \\
% % Ours-$\tilde{A}^g$ &   &   &   &   &   &   &   &   &   &   &   &   \\ 
% Ours &  710  &  \textbf{1553} & \textbf{1754} & \textbf{1638} & \underline{342}  & \textbf{874}  & \textbf{953}  &  \textbf{949} & \underline{106}  & \textbf{203}  &  \textbf{228} & \textbf{229}  \\
% \hline
% \end{tabular}
% \label{tbl:ablation-rmse}
% \end{table*}

==> tables/pcc+rmse.tex <==
\begin{table*}[t]
\footnotesize
\centering
\caption{RMSE and PCC performance of different methods on the three datasets with leadtime= 1, 5, 10, 15. Bold face indicates the best result of each column and underlined the second-best.}\label{table:all-rmse-pcc}
\scalebox{0.95}{\begin{tabular}{lcccccccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{Japan-Prefectures}} & \multicolumn{4}{c}{\textbf{US-Regions}} & \multicolumn{4}{c}{\textbf{US-States}} \\
\cmidrule(r){2-5}\cmidrule(r){6-9}\cmidrule(r){10-13}
% \rowcolor{grey!10}
\textbf{RMSE($\downarrow$)} & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 \\
\hline
GAR & 798 & 2426 & 2560 & 2477 & 358 & 1051 & 1492 & 1625 &  110& 247 & 340 & 368 \\
AR &999  & 2440 &2541  & 2474 &  377& 1075 & 1443 & 1546 &  120& 264 & 332 & 354 \\
VAR & 960 & 2568 & 2523 & 2344 & 447 &1094  & 1332 & 1381 & 285 & 317 & 433 & 435 \\
ARMA & 986 & 2439 & 2539 & 2248 & 377 & 1057 & 1426 & 1536 & 120 & 262 & 331 & 354 \\
% \hline
RNN & \textbf{695} & \underline{1710} & 1976 & 1903 & \underline{345} & \underline{953} & 1379 & 1556 & \underline{109} & \underline{224} &296  & 335 \\
RNN+Attn & 853 & 2184 & 1911 & 1957 & \underline{345} & 993 & 1378 & 1471 & 118 & 243 & 322 & 343 \\
CNNRNN-Res & 802 & 2248 & 2167 & 2097 & 421 & 972 & 1282 & 1361 & 140 & 293 & \underline{276} & \underline{274} \\
GCNRNN-Res & 829 & 1688 & \textbf{1675} & \underline{1681} & 631 & 987 & \underline{1135} & \underline{1029} & 187 & 274 & 314 & 314 \\
Cola-GNN &  \underline{710}  &  \textbf{1553} & \underline{1754} & \textbf{1638} & \textbf{342}  & \textbf{874}  & \textbf{953}  &  \textbf{949} & \textbf{106}  & \textbf{203}  &  \textbf{228} & \textbf{229}  \\
\midrule
% \textbf{PCC($\uparrow$)} & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} \\
% \rowcolor{grey!10}
\textbf{PCC($\uparrow$)}  & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 \\
\midrule
GAR & 0.9466  & 0.3202  &  0.3001  &  0.5456  &0.9734   &   0.7822 & 0.5686 &  0.4899 & 0.9715  &  0.86&  0.7253  & 0.6915  \\
AR & 0.9175 & 0.3022  & 0.36  & 0.5151 &  0.971 & 0.7884 & 0.6165 & 0.5579 & 0.9672  & 0.85  & 0.7391 & 0.6857 \\
VAR & 0.9216 &  0.229  & 0.2773  & 0.5221 &  0.9591  &  0.7258 & 0.563 &  0.5232 & 0.7976 & 0.7468 &  0.6069 &0.5154  \\
ARMA &  0.9182 & 0.3032 &  0.3655 & 0.445 & 0.9707  & 0.7864 & 0.6133 &  0.5547 & 0.9666  &  0.8498 &0.7383  &  0.6851\\
RNN & \textbf{0.9634}  & \underline{0.8038}  &  0.6874 &  0.7065 & \underline{0.9758} & \underline{0.8277} & 0.6435 & 0.5131 &  \underline{0.9733} &\underline{0.8919}  & 0.8013  & 0.7508   \\
RNN+Attn &  0.9518& 0.53 & 0.7309 &0.6825 & 0.9754  &  0.82 &  0.63 &  0.5905  &0.9701  & 0.8716 & 0.755 & 0.7238  \\
CNNRNN-Res & 0.9496   & 0.445 & 0.5857 &  0.5923 &  0.966 & 0.7899 & 0.6067  & 0.5535  &  0.9563  & 0.7887 & \underline{0.8224} & \underline{0.8337}  \\
GCNRNN-Res &  0.9533 & 0.7959 & \textbf{0.8203} & \underline{0.7847}  & 0.9226  & 0.8194  & \underline{0.7514} & \underline{0.7762} &  0.9176  & 0.8162 & 0.7728  &0.7731  \\
Cola-GNN & \underline{0.9622} &\textbf{ 0.84 } & \underline{0.7982} &  \textbf{0.7922} &  \textbf{0.976} &  \textbf{0.8548} & \textbf{0.8201}  & \textbf{0.8135}  &  \textbf{0.9745} &  \textbf{0.9121} & \textbf{0.8932} & \textbf{0.8927} \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/pcc.tex <==
\begin{table*}[]
\footnotesize
\centering
\caption{\footnotesize PCC performance of different methods on the three datasets with leadtime= 1, 5, 10, 15. Bold face indicates the best result of each column and underlined the second-best.}\label{table:all-pcc}
\begin{tabular}{|r|cccc|cccc|cccc|}
\hline
 & \multicolumn{4}{c|}{Japan-Prefectures} & \multicolumn{4}{c|}{US-Regions} & \multicolumn{4}{c|}{US-States} \\
Methods & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 \\
\hline
GAR & 0.9466  & 0.3202  &  0.3001  &  0.5456  &0.9734   &   0.7822 & 0.5686 &  0.4899 & 0.9715  &  0.86&  0.7253  & 0.6915  \\
AR & 0.9175 & 0.3022  & 0.36  & 0.5151 &  0.971 & 0.7884 & 0.6165 & 0.5579 & 0.9672  & 0.85  & 0.7391 & 0.6857 \\
VAR & 0.9216 &  0.229  & 0.2773  & 0.5221 &  0.9591  &  0.7258 & 0.563 &  0.5232 & 0.7976 & 0.7468 &  0.6069 &0.5154  \\
ARMA &  0.9182 & 0.3032 &  0.3655 & 0.445 & 0.9707  & 0.7864 & 0.6133 &  0.5547 & 0.9666  &  0.8498 &0.7383  &  0.6851\\
RNN & \textbf{0.9634}  & \underline{0.8038}  &  0.6874 &  0.7065 & \underline{0.9758} & \underline{0.8277} & 0.6435 & 0.5131 &  \underline{0.9733} &\underline{0.8919}  & 0.8013  & 0.7508   \\
RNN+Attn &  0.9518& 0.53 & 0.7309 &0.6825 & 0.9754  &  0.82 &  0.63 &  0.5905  &0.9701  & 0.8716 & 0.755 & 0.7238  \\
CNNRNN-Res & 0.9496   & 0.445 & 0.5857 &  0.5923 &  0.966 & 0.7899 & 0.6067  & 0.5535  &  0.9563  & 0.7887 & \underline{0.8224} & \underline{0.8337}  \\
GCNRNN-Res &  0.9533 & 0.7959 & \textbf{0.8203} & \underline{0.7847}  & 0.9226  & 0.8194  & \underline{0.7514} & \underline{0.7762} &  0.9176  & 0.8162 & 0.7728  &0.7731  \\
Ours & \underline{0.9622} &\textbf{ 0.84 } & \underline{0.7982} &  \textbf{0.7922} &  \textbf{0.976} &  \textbf{0.8548} & \textbf{0.8201}  & \textbf{0.8135}  &  \textbf{0.9745} &  \textbf{0.9121} & \textbf{0.8932} & \textbf{0.8927} \\
\hline
\end{tabular}
\end{table*}

==> tables/rmse.tex <==
\begin{table*}[]
\footnotesize
\centering
\caption{\footnotesize RMSE performance of different methods on the three datasets with leadtime= 1, 5, 10, 15. Bold face indicates the best result of each column and underlined the second-best.}\label{table:all-rmse}
\begin{tabular}{|r|cccc|cccc|cccc|}
\hline
 & \multicolumn{4}{c|}{Japan-Prefectures} & \multicolumn{4}{c|}{US-Regions} & \multicolumn{4}{c|}{US-States} \\
Methods & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 & 1 & 5 & 10 & 15 \\
\hline
GAR & 798 & 2426 & 2560 & 2477 & 358 & 1051 & 1492 & 1625 &  110& 247 & 340 & 368 \\
AR &999  & 2440 &2541  & 2474 &  377& 1075 & 1443 & 1546 &  120& 264 & 332 & 354 \\
VAR & 960 & 2568 & 2523 & 2344 & 447 &1094  & 1332 & 1381 & 285 & 317 & 433 & 435 \\
ARMA & 986 & 2439 & 2539 & 2248 & 377 & 1057 & 1426 & 1536 & 120 & 262 & 331 & 354 \\
\hline
RNN & \textbf{695} & \underline{1710} & 1976 & 1903 & \underline{345} & \underline{953} & 1379 & 1556 & \underline{109} & \underline{224} &296  & 335 \\
RNN+Attn & 853 & 2184 & 1911 & 1957 & \underline{345} & 993 & 1378 & 1471 & 118 & 243 & 322 & 343 \\
CNNRNN-Res & 802 & 2248 & 2167 & 2097 & 421 & 972 & 1282 & 1361 & 140 & 293 & \underline{276} & \underline{274} \\
GCNRNN-Res & 829 & 1688 & \textbf{1675} & \underline{1681} & 631 & 987 & \underline{1135} & \underline{1029} & 187 & 274 & 314 & 314 \\
Ours &  \underline{710}  &  \textbf{1553} & \underline{1754} & \textbf{1638} & \textbf{342}  & \textbf{874}  & \textbf{953}  &  \textbf{949} & \textbf{106}  & \textbf{203}  &  \textbf{228} & \textbf{229}  \\
\hline
\end{tabular}
\end{table*}
